Robust and structure exploiting optimization algorithms: An integral quadratic constraint approach

We consider the problem of analyzing and designing gradient-based discrete-time optimization algorithms for a class of unconstrained optimization problems having strongly convex objective functions with Lipschitz continuous gradient. By formulating the problem as a robustness analysis problem and making use of a suitable adaptation of the theory of integral quadratic constraints, we establish a framework that allows to analyze convergence rates and robustness properties of existing algorithms and enables the design of novel robust optimization algorithms with prespecified guarantees capable of exploiting additional structure in the objective function.

==> myStandardPreamble_arXiv.tex <==
% change @-symbol interpretation for using macros
\makeatletter

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% =============================
% ===         M I S C      ====
% =============================

% extended TeX
\@ifpackageloaded{etex}{}{\RequirePackage{etex}}

% etoolbox, useful for defining new commands
\@ifpackageloaded{etoolbox}{}{\RequirePackage{etoolbox}}

% keeps relative paths when including different .tex-files
% use \subimport*{subdirectory}{tex-File} to input tex-Files
\@ifpackageloaded{import}{}{\usepackage{import}}

% nice tables
\@ifpackageloaded{booktabs}{}{\usepackage{booktabs}}

% microtype for better spacing of letters
% \@ifpackageloaded{microtype}{}{\usepackage{microtype}}

% calculations also in tex-Code
\@ifpackageloaded{calc}{}{\usepackage{calc}}

% if conditions
\@ifpackageloaded{ifthen}{}{\usepackage{ifthen}}



% =============================
% ===    G R A P H I C S    ===
% =============================
\@ifpackageloaded{graphicx}{}{\usepackage{graphicx}}
\@ifpackageloaded{xcolor}{}{\usepackage{xcolor}}


% =============================
% ===         T I K Z      ====
% =============================
\@ifpackageloaded{tikz}{
     \usetikzlibrary{arrows,shapes,patterns,positioning,calc}
     }{
     \usepackage{tikz}
     \usetikzlibrary{arrows,shapes,patterns,positioning,calc}
}
\@ifpackageloaded{pgfplots}{
     }{
     \usepackage{pgfplots}
     }
% SOME TIKZ STYLE DEFINITIONS
\tikzstyle{boxstyle}=[draw=black,inner sep=7pt]      % style for boxes in blockdiagrams
\tikzstyle{arrowstyle}=[]                            % style for arrows in blockdiagrams



% =============================
% ===         M A T H      ====
% =============================
\@ifpackageloaded{amsmath}{}{\usepackage{amsmath}}
\@ifpackageloaded{amsfonts}{}{\usepackage{amsfonts}}
\@ifpackageloaded{amssymb}{}{\usepackage{amssymb}}
\let\theoremstyle\relax
\@ifpackageloaded{amsthm}{}{\usepackage{amsthm}}
\@ifpackageloaded{yhmath}{}{\usepackage{yhmath}}
\@ifpackageloaded{mathdots}{}{\usepackage{mathdots}}
\@ifpackageloaded{mathtools}{}{\usepackage{mathtools}}

% =============================
% ===    H Y P E R R E F    ===
% =============================

% some color definitions
\colorlet{lcolor}{green!45!black}
\colorlet{ucolor}{magenta!40!black}
\colorlet{ccolor}{green!40!black}

% hyperref for internal links
\usepackage[colorlinks=true,%
            linkcolor=lcolor,%
            urlcolor=lcolor,%
            citecolor=lcolor]{hyperref}

% cleverref for automatically labeling of references
\usepackage[nameinlink]{cleveref}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% rechange @-symbol interpretation
\makeatother


==> subfiles/overviewMatlabToolbox.tex <==
The presented design tools have been implemented in \textsc{Matlab}
using \textsc{Yalmip} 
The following list presents a brief overview of these function.
\paragraph{Algorithm analysis}
\begin{itemize}[leftmargin=*]
	\item \texttt{analyzeAlgoIQC} --
	      Check whether a given algorithm $ (\Aopt,\Bopt,\Copt,\Dopt) $ converges
	      with a specified convergence rate $\rho$ (\Cref{lemmaAnalysisConvRate}).
	\item \texttt{analyzeAlgoIQCPerf} --
	      Determine an upper bound on a performance measure ($H_2$ or $H_\infty$) of a given algorithm
	      $ (\Aopt,\Bopt,\Copt,\Dopt) $ with performance channel $ (\Bperf,\Cperf,\Dperf) $ (\Cref{lemmaAnalysisH2}, \Cref{lemmaAnalysisHinfty}).
	\item \texttt{getConvergenceRate} --
	      Get the best upper bound on the convergence rate of a given algorithm
	      $ (\Aopt,\Bopt,\Copt,\Dopt) $ by a bisection search and using \texttt{analyzeAlgoIQC}.
\end{itemize}
\paragraph{Algorithm synthesis}
\begin{itemize}[leftmargin=*]	
	\item \texttt{synthesizeAlgoIQCconservative} --
	      Design an algorithm $ (\Aopt,\Bopt,\Copt,\Dopt) $ with prespecified
	      or optimal convergence rate $ \rho $ using the conservative convex approach
	      (\Cref{lemmaConservativeConvexSynthesisNew}).
	\item \texttt{synthesizeAlgoIQCconservativePerf} --
	      Design an algorithm $ (\Aopt,\Bopt,\Copt,\Dopt) $ with prespecified or optimal
	      convergence rate $ \rho $ and optimal $H_2$-performance bound 
	      using the conservative convex approach 
	      (\Cref{lemmaConservativeConvexSynthesisWithPerf}).
	\item \texttt{snythesizeAlgoIQClocalBMI} -- 
	      Design an algorithm $ (\Aopt,\Bopt,\Copt,\Dopt) $ with prespecified or optimal
	      convergence rate $ \rho $ using a BMI optimization approach.
	\item \texttt{synthesizeAlgoIQClocalBMIperf} --
	      Design an algorithm $ (\Aopt,\Bopt,\Copt,\Dopt) $ with prespecified or optimal
	      convergence rate $ \rho $ and optimal $H_2$-performance bound 
	      using a BMI optimization approach.
	\item \texttt{getControllerViaSProcedure} --
	      Design a structured algorithm $ (\Aopt,\Bopt,\Copt,\Dopt) $ with prespecified
	      convergence rate $ \rho $ using the approach described in~\Cref{secAppendixDesignStructuredAlgorithms}.
\end{itemize}
\paragraph{Low level functions}
\begin{itemize}[leftmargin=*]
	\item \texttt{getIqcDelta} --
	      Returns the IQC for exponential convergence for the uncertainty $ \Delta $.
	\item \texttt{getIqcPerf} --
	      Returns the performance IQC multiplier.
	\item \texttt{getConvRateLMI} --
	      Returns the convergence LMIs as an \texttt{sdpvar} object.
	\item \texttt{getPerfLMI} --
	      Returns the performance LMIs as an \texttt{sdpvar} object.
	\item \texttt{synthesizeAlgoIQCfixedP} --
	      Solve the synthesis LMIs for fixed $P$. Used in alternating approach for BMI optimization.
	\item \texttt{generateRandomFunction} --
	      Generate a random function from the class $ S_{m,L}^2 $.
\end{itemize}
\paragraph{State-space representations}
\begin{itemize}[leftmargin=*]
	\item \texttt{getAlgorithm} --
	      Returns a state-space representation of some important algorithms
	      such as \nesterov, \gradDesc, the \heavyBall{} or the \tripleMomentum.
	\item \texttt{ss2ssStruct} --
	      Transform a \textsc{Matlab} \texttt{ss} object to a struct with 
	      data fields $ A, B, C, D $.
	\item \texttt{ssStructSeries} --
	      State-space representation of the series connection of two 
	      state-space representations saved in structs.
	\item \texttt{transformToCanonical} --
	      Transform a given algorithm $ ( \Aopt,\Bopt,\Copt,\Dopt ) $
	      to the canonical form as given in~\Cref{secAppendixDesignStructuredAlgorithms}.
\end{itemize}
\paragraph{Visualization}
\begin{itemize}[leftmargin=*]
	\item \texttt{setPlotStyle} --
	      Set the style of a line to some predefined sets of values.
\end{itemize}
\paragraph{Examples}
\begin{itemize}[leftmargin=*]
	\item \texttt{analysisOfExistingAlgorithmsConvRate} --
	      Analyze the convergence rates of \nesterov, \gradDesc, 
	      the \heavyBall{} and the \tripleMomentum{} using~\Cref{lemmaAnalysisConvRate}.
	      This produces~\Cref{figConvRatesAnalysis}.
	\item \texttt{perfAnalysisExistingAlgos} --
	      Analyze the $H_2$-performance (and also $H_\infty$-performance)
	      of \nesterov, \gradDesc, the \heavyBall{} and the \tripleMomentum{}
	      using~\Cref{lemmaAnalysisH2}, \Cref{lemmaAnalysisHinfty}.
	      This produces~\Cref{figH2Analysis}.
	\item \texttt{examplePaper\_simNoise} --
	      Analyze the $H_2$-performance using a sample-based approach.
	      This produces\ifthenelse{\boolean{singleColumn}}{~\Cref{figH2Analysis}}{~\Cref{figH2AnalysisSampleBased}}.
\end{itemize}

